Delay-Tolerant Networking for Long-Term Animal Tracking

Enabling Internet connectivity for mobile objects that do not have a permanent home or regular movements is a challenge due to their varying energy budget, intermittent wireless connectivity, and inaccessibility. We present a hardware and software framework that offers robust data collection, adaptive execution of sensing tasks, and flexible remote reconfiguration of devices deployed on nomadic mobile objects such as animals. The framework addresses the overall complexity through a multi-tier architecture with low tier devices operating on a tight energy harvesting budget and high tier cloud services offering seamless delay-tolerant presentation of data to end users. Based on our multi-year experience of applying this framework to animal tracking and monitoring applications, we present the main challenges that we have encountered, the design of software building blocks that address these challenges, and examples of the data we collected on flying foxes.

==> biographies.tex <==
% !TEX root = paper.tex
\section*{Biographies}

\textbf{Philipp Sommer}, Postdoctoral Fellow, CSIRO, Autonomous Systems, Brisbane, Australia. E-mail: philipp.sommer@csiro.au.\\
\\
\textbf{Brano Kusy}, Principal Research Scientist, CSIRO, Autonomous Systems, Brisbane, Australia. E-mail: brano.kusy@csiro.au.\\
\\
\textbf{Philip Valencia}, Software Engineer, CSIRO, Autonomous Systems, Brisbane, Australia. E-mail: philip.valencia@csiro.au.\\
\\
\textbf{Ross Dungavell}, Senior Software Engineer, CSIRO, Autonomous Systems, Brisbane, Australia. E-mail: ross.dungavell@csiro.au.\\
\\
\textbf{Raja Jurdak}, Principal Research Scientist, CSIRO, Autonomous Systems, Brisbane, Australia. E-mail: raja.jurdak@csiro.au.
